Scale-Aware Recognition in Satellite Images under Resource Constraints

Recognition of features in satellite imagery (forests, swimming pools, etc.) depends strongly on the spatial scale of the concept and therefore the resolution of the images. This poses two challenges: Which resolution is best suited for recognizing a given concept, and where and when should the costlier higher-resolution (HR) imagery be acquired? We present a novel scheme to address these challenges by introducing three components: (1) A technique to distill knowledge from models trained on HR imagery to recognition models that operate on imagery of lower resolution (LR), (2) a sampling strategy for HR imagery based on model disagreement, and (3) an LLM-based approach for inferring concept "scale". With these components we present a system to efficiently perform scale-aware recognition in satellite imagery, improving accuracy over single-scale inference while following budget constraints. Our novel approach offers up to a 26.3% improvement over entirely HR baselines, using 76.3% fewer HR images.

==> figures/HR_LR_example.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5 \columnwidth]{images/HRLRexample.png}
    \caption{Example of LR Image (left) and the HR images which cover the same region (right).}
    \label{fig:HR_LR_example}
\end{figure}

==> figures/Intro_figure.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.9 \columnwidth]{images/Title Figure Sized.png}
    \caption{Images of the same region in two resolutions. On the right we have images from Sentinel-2, where the spatial resolution of one pixel corresponds to 10 meters on the ground. On the left we have the corresponding NAIP images, where the spatial resolution of one pixel corresponds to 1 meter on the ground. With the task of concept recognition, we can see that different resolutions are better suited to different tasks. For example if we were looking to recognize a large concept such as a forest, a lower resolution image is better suited as we can see from (a) and (c), a park in a developed town can appear similar to a forest at a high resolution, as we cannot immediately see the surrounding context. If we were looking to recognize an American football field, we would prefer a higher resolution image, as one can see from (b) and (d), that some concepts cannot be perceived at a low resolution. }
    \label{fig:Title_Figure}
\end{figure}

==> figures/KD_figure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5 \columnwidth]{graph-placeholder.jpg}
    \caption{Visualization demonstrating improvement in concept detection with KD.}
    \label{fig:knowledge_distill}
\end{figure}

==> figures/LLM.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5 \columnwidth]{graph-placeholder.jpg}
    \caption{Concept detection performance comparison between resolution-selected models (HR vs. LR)}
    \label{fig:LLM}
\end{figure}

==> tables/rebuttal_overall_with_runtime.tex <==
\begin{table}[ht]
    \centering
    \scalebox{0.8}{
   \begin{tabular}{lccc}
   \toprule
        Model & mAP & HR images acquired in Million sq. km. & runtime in s\\
       \hline \\
       \textcolor{gray}{GRAFT HR} & \textcolor{gray}{0.432}  & \textcolor{gray}{25163.2} & \textcolor{gray}{1539.22}\\
        GRAFT LR &  0.343 & 0 &  17.054\\
        GRAFT KD &  0.375  & 0 & 17.071\\
        GRAFT LR + nl. sampling~\cite{meng2022count} & 0.358 & \textbf{5953.6} & 322.811\\
        GRAFT KD + HR & 0.418  & \textbf{5953.6} & 339.882\\
        GRAFT LR + LLM & 0.433 & 25163.2 & 1575.429\\
        GRAFT KD + LLM  & 0.433  & 25163.2 & 1569.640 \\
        \textbf{Ours full (GRAFT)} & \textbf{0.460} & \textbf{5953.6} & 372.370 \\
        
        
        \\
         \textcolor{gray}{Resnet 50 HR} & \textcolor{gray}{0.424} & \textcolor{gray}{25163.2} & \textcolor{gray}{1585.395}\\
        Resnet 50 LR & 0.389 & 0 &  13.710\\
        Resnet 50 KD & 0.428 & 0 & 13.668 \\
        ResNet-50 LR + LLM & 0.439 & 25163.2 & 1609.535\\
        ResNet-50 KD + HR &  0.419 & \textbf{5953.6} & 327.532 \\
        ResNet-50 KD+ LLM &  0.428 & 25163.2 & 1609.493\\
        \textbf{Ours full (Resnet-50)} &  \textbf{0.457} & \textbf{5953.6} & 337.962 \\
        \\
      \textcolor{gray}{Satlas HR} & \textcolor{gray}{0.309} & \textcolor{gray}{25163.2} & \textcolor{gray}{1736.692}\\
        Satlas LR & 0.307 & 0 & 15.837\\
        Satlas KD & 0.310 & 0 & 15.388\\
        SATLAS + LLM & 0.325 & 25163.2 & 1762.959\\
        SATLAS + HR & 0.310 &\textbf{5953.6} & 337.182\\
        SATLAS KD + LLM & 0.317 & 25163.2 & 1762.510\\
        \textbf{Ours full (Satlas)} & \textbf{0.326} & \textbf{5953.6} & 347.612 \\ 

        \hline 
        \\
        Resnet 50 (Multi-Res) & 0.376 & 0 & 21.236 \\
        Scalemae~\cite{reed2023scale} & 0.371& 0 &61.186 \\
        Satmae~\cite{cong-22} & 0.355& 0 & 67.051 \\
        Cross-Scale MAE~\cite{tang2023cross} & 0.388 & 0 & 90.702\\
        Patchdrop~\cite{uzkent2020learning} & 0.442   & 6775.8 & 359.779 \\
        \bottomrule
    \end{tabular}
        }
    \caption{Full system performance under various settings for retrieval under budget. For models using both HR and LR data, we assign a budget of 1000 locations (each corresponding to about 5 sq. kms) per concept. The runtime is calculated on our test set of 5015 images, for a batch size of 32 on a single Nvidia RTX A6000 GPU. Our full system can perform much better that the baselines with improved HR data budget constraints.}
    \label{tab:overall_rebuttal}
\end{table}



==> tables/rebuttal_train_times.tex <==
\begin{table}[h]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{cc}
        Model & Training time for 200 epochs (hours) \\
        \hline
        \\
        GRAFT KD &  36.76\\
        ResNet 50 KD & 11.23\\
        Satlas 50 KD & 24.98 \\
    \end{tabular}
    }
    \caption{Models and their respective training times for 200 epochs. All KD models were trained on a single Nvidia RTX A6000 GPU.}
    \label{tab:Train_Times}
\end{table}
